Speech-Based Parameter Estimation of an Asymmetric Vocal Fold Oscillation Model and Its Application in Discriminating Vocal Fold Pathologies

So far, several physical models have been proposed for the study of vocal fold oscillations during phonation. The parameters of these models, such as vocal fold elasticity, resistance, etc. are traditionally determined through the observation and measurement of the vocal fold vibrations in the larynx. Since such direct measurements tend to be the most accurate, the traditional practice has been to set the parameter values of these models based on measurements that are averaged across an ensemble of human subjects. However, the direct measurement process is hard to revise outside of clinical settings. In many cases, especially in pathological ones, the properties of the vocal folds often deviate from their generic values---sometimes asymmetrically wherein the characteristics of the two vocal folds differ for the same individual. In such cases, it is desirable to find a more scalable way to adjust the model parameters on a case by case basis. In this paper, we present a novel and alternate way to determine vocal fold model parameters from the speech signal. We focus on an asymmetric model and show that for such models, differences in estimated parameters can be successfully used to discriminate between voices that are characteristic of different underlying vocal fold pathologies.

==> IEEEtrans_package/README <==

September 17, 2014


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8a has a number of significant changes over the v1.8 release.
For a full list of changes, please read the file changelog.txt. The most
notable changes include:


 1) Extensive rework of the compsoc mode to comply with the latest standards
    of the IEEE Computer Society.

 2) Fixed abstract, index terms and diamond line for compsoc technotes.

 3) New \IEEEraisesectionheading{} command to provide for the special
    raised first section heading of Computer Society journal papers.

 4) Internal code improvements for page setup and command argument
    processing.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_compsoc.tex, bare_jrnl_transmag.tex
***************************************************************************


==> backup.tex <==
FROM INTRO:

Phonation is the process wherein the vocal folds in the larynx are set into a state of self-sustained vibration, causing an excitation signal to be produced at the glottal source. This signal resonates in the vocal tract of the speaker, and depending on the shape of the vocal tract and the configuration of the articuclators (tongue, lip, jaw etc.), is heard as a characteristic voiced sound by the listener. Phonation is thus important in the production of all vowels and all voiced consonants in all languages of the world.

%The oscillation of the vocal folds is fundamental to phonation. During phonation, the airstream from lungs is modulated by the displacement of vocal folds, creating a glottal flow pattern~\cite{titze1988physics} that produces the fundamental frequency of voicing. The dynamic interaction of the glottal flow with the vocal tract generates different speech tones. 

The self-sustained vibrations of the vocal folds are conjectured to be initiated and driven by a delicate balance of physical and hydrodynamic forces across the glottis, in which the muscles of the larynx and the dynamics of the airflow across it play a critical role.
The exact physics of the airflow through the glottis during phonation is well studied, e.g.,~\cite{flanagan1968self,ishizaka1972synthesis,titze1988physics,zhang2006influence,zhao2002computational,zhang2002computational}, and a number of physical models have been proposed for it
%. Based on an understanding of this process, several physical models have been proposed in literature that attempt to emulate the phonation process 
e.g.,~\cite{ishizaka1972synthesis,lucero1993dynamics, lucero2013modeling,alipour2000finite,yang2011computation,pickup2009influence}.
%Each such model uses measured bio-mechanical properties of the vocal folds within a set of dynamically solvable equations that capture the balance of forces across the glottis during phonation. The output of each model is a trajectory in two or three-dimensional space that represents the self-sustained motion of the vocal folds.
The models use measured bio-mechanical properties of the vocal folds, such as vocal-fold elasticity and resistance, within a set of dynamical equations which capture the movements of the glottis during phonation. 
%The model output is a trajectory in two or three-dimensional space that represents the self-sustained motion of the vocal folds.

The properties of the vocal structures vary from their generic settings in pathological cases such as vocal palsy, phonotrauma, neoplasm, etc~\cite{bhat2018femh}. In these cases, the movements of the vocal folds are frequently observed to be asymmetric~\cite{steinecke1995bifurcations}; in fact their pattern of movement is often a signature of the underlying pathology. To explain these, {\em asymmetric} dynamical models of the vocal folds have been proposed that are able to emulate these asymmetric vibratory motions of the vocal folds~\cite{erath2006investigation}, by appropriate setting of their parameters.

While the \textit{forward} problem of accurately emulating vocal fold movements during phonation is effectively solved by these models, the \textit{reverse} problem of finding the correct model parameters given a set of observed vocal fold movements has not been addressed. The primary objective of this paper is to present this reverse problem, and suggest a methodology to solve it based on analysis of the speech signal. Given a model for asymmetric movements of the vocal folds and a set of speech signals from people affected by various pathologies which affect vocal fold movements, we propose a method to estimate the parameters of the asymmetric model that explains them.

We further show how the re-estimated model parameters can be mapped into the phase space of the nonlinear dynamical systems that represent the asymmetric model, and how the location of these parameters in the phase space of the model can directly indicate the underlying pathology that the observed speech signal represents.
